No way ou$\tau$: Epoch of Reionization Observations Do not Support Large Values of the Optical Depth to Reionization

Recent cosmological analyses combining high-redshift cosmic microwave background (CMB) measurements with low-redshift baryon acoustic oscillation (BAO) data have reported a preference for dynamical dark energy, with the cosmological constant scenario ($\Lambda$CDM) disfavored at the $\sim 3\sigma$ level. These analyses, however, typically rely on large-scale CMB polarization measurements to constrain the optical depth to reionization $\tau_{\rm reio}\sim 0.06$, raising the question of whether potential systematics in this dataset could influence the inferred cosmological preference. Excluding large-scale polarization data substantially weakens the tension with $\Lambda$CDM to the $\lesssim 2\sigma$ level, nevertheless at a price of increasing $\tau_{\rm reio}$ significantly to $\sim 0.09$. Here, we use a physically motivated Gompertzian reionization framework to perform a self-consistent Bayesian analysis combining CMB (excluding large-scale polarization data), BAO, and independent measurements of the neutral hydrogen fraction evolution from quasar damping wing observations and dark pixel constraints. We derive $\tau_{\rm reio} = 0.067 \pm 0.011$ (dynamical dark energy scenario) in good agreement with cosmological analyses that would include large-scale CMB polarization data, while the inferred reionization history is consistent with multiple observational constraints. Our analysis recovers a preference for dynamical dark energy at the $\gtrapprox2\sigma$ level. These results demonstrate that astrophysical probes of reionization independently recover the optical depth required by CMB polarization measurements, suggesting that potential systematics in large-scale polarization alone are unlikely to fully explain the emerging preference for dynamical dark energy.

==> define.tex <==
%--------------- User Defined Commands ---------------------%
% Journals 
% Bibliography and bibfile
\def\aj{AJ}%
          % Astronomical Journal
\def\actaa{Acta Astron.}%
          % Acta Astronomica
\def\araa{ARA\&A}%
          % Annual Review of Astron and Astrophys
\def\apj{ApJ}%
          % Astrophysical Journal
\def\apjl{ApJ}%
          % Astrophysical Journal, Letters
\def\apjs{ApJS}%
          % Astrophysical Journal, Supplement
\def\ao{Appl.~Opt.}%
          % Applied Optics
\def\apss{Ap\&SS}%
          % Astrophysics and Space Science
\def\aap{A\&A}%
          % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}%
          % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}%
          % Astronomy and Astrophysics, Supplement
\def\azh{AZh}%
          % Astronomicheskii Zhurnal
\def\baas{BAAS}%
          % Bulletin of the AAS
\def\bac{Bull. astr. Inst. Czechosl.}%
          % Bulletin of the Astronomical Institutes of Czechoslovakia 
\def\caa{Chinese Astron. Astrophys.}%
          % Chinese Astronomy and Astrophysics
\def\cjaa{Chinese J. Astron. Astrophys.}%
          % Chinese Journal of Astronomy and Astrophysics
\def\icarus{Icarus}%
          % Icarus
\def\jcap{J. Cosmology Astropart. Phys.}%
          % Journal of Cosmology and Astroparticle Physics
\def\jrasc{JRASC}%
          % Journal of the RAS of Canada
\def\mnras{MNRAS}%
          % Monthly Notices of the RAS
\def\memras{MmRAS}%
          % Memoirs of the RAS
\def\na{New A}%
          % New Astronomy
\def\nar{New A Rev.}%
          % New Astronomy Review
\def\pasa{PASA}%
          % Publications of the Astron. Soc. of Australia
\def\pra{Phys.~Rev.~A}%
          % Physical Review A: General Physics
\def\prb{Phys.~Rev.~B}%
          % Physical Review B: Solid State
\def\prc{Phys.~Rev.~C}%
          % Physical Review C
\def\prd{Phys.~Rev.~D}%
          % Physical Review D
\def\pre{Phys.~Rev.~E}%
          % Physical Review E
\def\prl{Phys.~Rev.~Lett.}%
          % Physical Review Letters
\def\pasp{PASP}%
          % Publications of the ASP
\def\pasj{PASJ}%
          % Publications of the ASJ
\def\qjras{QJRAS}%
          % Quarterly Journal of the RAS
\def\rmxaa{Rev. Mexicana Astron. Astrofis.}%
          % Revista Mexicana de Astronomia y Astrofisica
\def\skytel{S\&T}%
          % Sky and Telescope
\def\solphys{Sol.~Phys.}%
          % Solar Physics
\def\sovast{Soviet~Ast.}%
          % Soviet Astronomy
\def\ssr{Space~Sci.~Rev.}%
          % Space Science Reviews
\def\zap{ZAp}%
          % Zeitschrift fuer Astrophysik
\def\nat{Nature}%
          % Nature
\def\iaucirc{IAU~Circ.}%
          % IAU Cirulars
\def\aplett{Astrophys.~Lett.}%
          % Astrophysics Letters
\def\apspr{Astrophys.~Space~Phys.~Res.}%
          % Astrophysics Space Physics Research
\def\bain{Bull.~Astron.~Inst.~Netherlands}%
          % Bulletin Astronomical Institute of the Netherlands
\def\fcp{Fund.~Cosmic~Phys.}%
          % Fundamental Cosmic Physics
\def\gca{Geochim.~Cosmochim.~Acta}%
          % Geochimica Cosmochimica Acta
\def\grl{Geophys.~Res.~Lett.}%
          % Geophysics Research Letters
\def\jcp{J.~Chem.~Phys.}%
          % Journal of Chemical Physics
\def\jgr{J.~Geophys.~Res.}%
          % Journal of Geophysics Research
\def\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\def\memsai{Mem.~Soc.~Astron.~Italiana}%
          % Mem. Societa Astronomica Italiana
\def\nphysa{Nucl.~Phys.~A}%
          % Nuclear Physics A
\def\physrep{Phys.~Rep.}%
          % Physics Reports
\def\physscr{Phys.~Scr}%
          % Physica Scripta
\def\planss{Planet.~Space~Sci.}%
          % Planetary Space Science
\def\procspie{Proc.~SPIE}%
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

% Song Huang's definition 
\def\arcsec{{\prime\prime}}
\def\arcmin{{\prime}}
\def\degree{{\circ}}
\def\h{\hskip -3 mm}
\def\amin{$^\prime$}
\def\asec{$^{\prime\prime}$}
\def\deg{$^{\circ}$}
\def\ddeg{{\rlap.}$^{\circ}$}
\def\dsec{{\rlap.}$^{\prime\prime}$}
\def\cc{cm$^{-3}$}
\def\flamb{erg s$^{-1}$ cm$^{-2}$ \AA$^{-1}$}
\def\flux{erg s$^{-1}$ cm$^{-2}$}
\def\fnu{erg s$^{-1}$ cm$^{-2}$ Hz$^{-1}$}
\def\kms{km s$^{-1}$}
\def\lamb{$\lambda$}
\def\micron{{$\mu$m}}
\def\perang{\AA$^{-1}$}
\def\peryr{yr$^{-1}$}
\def\lsun{$L_\odot$} 
\def\sigs{$\sigma_*$}
\def\etal{{\ et al.}}
\def\mpch{$\,h^{-1}\,{\rm Mpc}$}
\def\hmpc{$\,h\,{\rm Mpc}^{-1}$}
\newcommand{\lt}{<}
\newcommand{\gt}{>}

% wenting's definition
\newcommand{\ww}[1]{\textcolor{magenta}{{#1}}}
\newcommand{\msun}{\mathrm{M}_\odot}


% ----- Editing and commenting ----- %
% Color
\definecolor{LightGray}{gray}{0.85}
\definecolor{Tab1}{RGB}{114, 158, 206}
\definecolor{Tab2}{RGB}{255, 158,  74}
\definecolor{Tab3}{RGB}{103, 191,  92}
\definecolor{Tab4}{RGB}{174, 199, 232}
\definecolor{Tab5}{RGB}{255, 187, 120}
\definecolor{Tab6}{RGB}{152, 223, 138}
\definecolor{Tab7}{RGB}{255, 152, 150}
\definecolor{Tab8}{RGB}{197, 176, 213}
\definecolor{hpurple}{HTML}{7E16DF}

% Commenting:
\newcommand{\todo}[1]{\textcolor{BrickRed}{\textbf{~#1}}} % Todo list
\newcommand{\plan}[1]{\textcolor{Sepia}{#1}} % Plan for the draft
\newcommand{\addref}{{\textcolor{red}{ADDREF}}} % Need to add refereces
\newcommand{\update}[1]{\textcolor{PineGreen}{#1}} % Updated text
\newcommand{\code}[1]{\textbf{\texttt{#1}}} % Code or software name
\newcommand{\temp}[1]{\textcolor{OliveGreen}{#1}} % For placeholder

% For different comments
\newcommand{\note}[2]{\textcolor{blue}{\textbf{[Comment (#1): #2]}}}
\newcommand{\cheng}[1]{\textcolor{blue}{\textbf{[Cheng: #1]}}}
\newcommand{\song}[1]{\textcolor{Cyan}{\textbf{[Song: #1]}}}
\newcommand{\paulo}[1]{{\textcolor{cyan}{[PMC: #1]}}}
\newcommand{\yao}[1]{{\textcolor{red}{[YZ: #1]}}}
\newcommand{\jiaxi}[1]{{\textcolor{olive}{[jiaxi: #1]}}}
\newcommand{\pablo}[1]{{\textcolor{orange}{[PRG: #1]}}}
\newcommand{\siyi}[1]{{\textcolor{orange}{[Siyi: #1]}}}
\newcommand{\zhiqi}[1]{{\textcolor{magenta}{[Zhiqi:#1]}}}
\newcommand{\xiaodong}[1]{{\textcolor{green}{[XD: #1]}}}
\newcommand{\jpk}[1]{{\textcolor{red}{[JPK: #1]}}}
\newcommand{\yucheng}[1]{{\textcolor{purple}{[Yucheng: #1]}}}
\newcommand{\rafaela}[1]{{\textcolor{olive}{[rafaela: #1]}}}
\newcommand{\outdated}[1]{{\color{gray}#1}}
\newcommand{\yunyi}[1]{{\color{magenta}Yunyi: #1}}
\newcommand{\wenshuo}[1]{{\textcolor{orange}{[wenshuo: #1]}}}

\newcommand{\AR}[1]{{\textcolor{BrickRed}{[Antoine: #1]}}}

%\DeclareRobustCommand{\ion}[2]{%
%\relax\ifmmode
%\ifx\testbx\f@series
%{\mathbf{#1\,\mathsc{#2}}}\else
%{\mathrm{#1\,\mathsc{#2}}}\fi
%\else\textup{#1\,{\mdseries\textsc{#2}}}%
%\fi}
